Parameterized Synthesis Case Study: AMBA AHB

We revisit the AMBA AHB case study that has been used as a benchmark for several reactive synthesis tools. Synthesizing AMBA AHB implementations that can serve a large number of masters is still a difficult problem. We demonstrate how to use parameterized synthesis in token rings to obtain an implementation for a component that serves a single master, and can be arranged in a ring of arbitrarily many components. We describe new tricks - property decompositional synthesis, and direct encoding of simple GR(1) - that together with previously described optimizations allowed us to synthesize a component model with 14 states in about 1 hour.

==> eptcsdata.tex <==
\providecommand{\firstpage}{68}
\providecommand{\publicationstatus}{K. Chatterjee, R. Ehlers, and S. Jha (Eds.): \\
Third Workshop on Synthesis (SYNT 2014)\\
EPTCS 157, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.157.9}{10.4204/EPTCS.157.9}}
\pdfoutput=1

